Volumetric Objectives for Multi-Robot Exploration of Three-Dimensional Environments

Volumetric objectives for exploration and perception tasks seek to capture a sense of value (or reward) for hypothetical observations at one or more camera views for robots operating in unknown environments. For example, a volumetric objective may reward robots proportionally to the expected volume of unknown space to be observed. We identify connections between existing information-theoretic and coverage objectives in terms of expected coverage, particularly that mutual information without noise is a special case of expected coverage. Likewise, we provide the first comparison, of which we are aware, between information-based approximations and coverage objectives for exploration, and we find, perhaps surprisingly, that coverage objectives can significantly outperform information-based objectives in practice. Additionally, the analysis for information and coverage objectives demonstrates that Randomized Sequential Partitions -- a method for efficient distributed sensor planning -- applies for both classes of objectives, and we provide simulation results in a variety of environments for as many as 32 robots.

==> fig/rate_by_environment/thesis_experiments_complete_coverage_rate_2420f96.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0,0.811764705882353,1}
\definecolor{color0}{rgb}{0.12156862745098,0.227450980392157,0.00392156862745098}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Num. Robots},
xmin=2.6, xmax=33.4,
xtick style={color=black},
xtick={4,8,16,32},
xmajorgrids,
y grid style={lightgray!92.0261437908!black},
ylabel={Coverage Rate (cells per robot-iteration)},
ymin=0, ymax=650,
ymajorgrids,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,257.670204611356)
--(axis cs:8,243.976272853769)
--(axis cs:16,207.936011185539)
--(axis cs:32,147.458998497086)
--(axis cs:32,143.167144754322)
--(axis cs:16,202.415816656055)
--(axis cs:8,235.660118404513)
--(axis cs:4,245.471262789259)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,280.219068084581)
--(axis cs:8,261.690157983634)
--(axis cs:16,198.656318618724)
--(axis cs:32,123.046330430952)
--(axis cs:32,120.094968737951)
--(axis cs:16,191.748822303584)
--(axis cs:8,253.734898781846)
--(axis cs:4,267.962373888143)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,254.168720814)
--(axis cs:8,253.374506496521)
--(axis cs:16,249.938996041713)
--(axis cs:32,220.213775616902)
--(axis cs:32,217.298039757092)
--(axis cs:16,243.021526021548)
--(axis cs:8,243.851845199274)
--(axis cs:4,242.046378781803)
--cycle;
\path [draw=color0, fill=color0, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,426.595007780432)
--(axis cs:8,424.246246758241)
--(axis cs:16,327.126079143829)
--(axis cs:32,203.666700149102)
--(axis cs:32,201.463355842485)
--(axis cs:16,320.607118648181)
--(axis cs:8,414.101187867669)
--(axis cs:4,417.629463744652)
--cycle;
\path [draw=color1, fill=color1, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,204.856174218076)
--(axis cs:8,222.761597892528)
--(axis cs:16,201.324039693759)
--(axis cs:32,141.323208531933)
--(axis cs:32,137.336065599296)
--(axis cs:16,194.697378001495)
--(axis cs:8,212.013149319567)
--(axis cs:4,188.540069892342)
--cycle;
\path [draw=orange, fill=orange, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,279.228108960923)
--(axis cs:8,289.342197822781)
--(axis cs:16,241.602010002165)
--(axis cs:32,171.919417329469)
--(axis cs:32,169.353781892773)
--(axis cs:16,225.515634487392)
--(axis cs:8,280.783448902937)
--(axis cs:4,219.674943290022)
--cycle;
\addplot [semithick, blue, dash pattern=on 3.7pt off 1.6pt]
table {%
4 251.570733700307
8 239.818195629141
16 205.175913920797
32 145.313071625704
};
\addplot [semithick, red, dash pattern=on 3.7pt off 1.6pt]
table {%
4 274.090720986362
8 257.71252838274
16 195.202570461154
32 121.570649584452
};
\addplot [semithick, green, dash pattern=on 3.7pt off 1.6pt]
table {%
4 248.107549797901
8 248.613175847897
16 246.480261031631
32 218.755907686997
};
\addplot [semithick, color0, dash pattern=on 3.7pt off 1.6pt]
table {%
4 422.112235762542
8 419.173717312955
16 323.866598896005
32 202.565027995793
};
\addplot [semithick, color1, dash pattern=on 3.7pt off 1.6pt]
table {%
4 196.698122055209
8 217.387373606048
16 198.010708847627
32 139.329637065615
};
\addplot [semithick, orange, dash pattern=on 3.7pt off 1.6pt]
table {%
4 249.451526125472
8 285.062823362859
16 233.558822244779
32 170.636599611121
};
\end{axis}

\end{tikzpicture}


==> fig/rate_by_environment/thesis_experiments_complete_coverage_rate_per_iteration_2420f96.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0,0.811764705882353,1}
\definecolor{color0}{rgb}{0.12156862745098,0.227450980392157,0.00392156862745098}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Num. Robots},
xmajorgrids,
xmin=2.6, xmax=33.4,
xtick style={color=black},
xtick={4,8,16,32},
y grid style={lightgray!92.0261437908!black},
ylabel={Coverage Rate (cells per iteration)},
ymajorgrids,
ymin=0, ymax=12000,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.2, line width=0.0pt]
(axis cs:4,1030.68081844542)
--(axis cs:8,1951.81018283015)
--(axis cs:16,3326.97617896863)
--(axis cs:32,4718.68795190675)
--(axis cs:32,4581.3486321383)
--(axis cs:16,3238.65306649687)
--(axis cs:8,1885.28094723611)
--(axis cs:4,981.885051157037)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0.0pt]
(axis cs:4,1120.87627233832)
--(axis cs:8,2093.52126386907)
--(axis cs:16,3178.50109789958)
--(axis cs:32,3937.48257379047)
--(axis cs:32,3843.03899961445)
--(axis cs:16,3067.98115685735)
--(axis cs:8,2029.87919025477)
--(axis cs:4,1071.84949555257)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0.0pt]
(axis cs:4,1016.674883256)
--(axis cs:8,2026.99605197217)
--(axis cs:16,3999.02393666741)
--(axis cs:32,7046.84081974086)
--(axis cs:32,6953.53727222694)
--(axis cs:16,3888.34441634477)
--(axis cs:8,1950.81476159419)
--(axis cs:4,968.185515127211)
--cycle;
\path [draw=color0, fill=color0, opacity=0.2, line width=0.0pt]
(axis cs:4,1706.38003112173)
--(axis cs:8,3393.96997406593)
--(axis cs:16,5234.01726630126)
--(axis cs:32,6517.33440477127)
--(axis cs:32,6446.82738695951)
--(axis cs:16,5129.71389837089)
--(axis cs:8,3312.80950294136)
--(axis cs:4,1670.51785497861)
--cycle;
\path [draw=color1, fill=color1, opacity=0.2, line width=0.0pt]
(axis cs:4,819.424696872304)
--(axis cs:8,1782.09278314023)
--(axis cs:16,3221.18463510014)
--(axis cs:32,4522.34267302187)
--(axis cs:32,4394.75409917748)
--(axis cs:16,3115.15804802391)
--(axis cs:8,1696.10519455653)
--(axis cs:4,754.160279569368)
--cycle;
\path [draw=orange, fill=orange, opacity=0.2, line width=0.0pt]
(axis cs:4,1116.91243584369)
--(axis cs:8,2314.73758258225)
--(axis cs:16,3865.63216003465)
--(axis cs:32,5501.42135454299)
--(axis cs:32,5419.32102056875)
--(axis cs:16,3608.25015179828)
--(axis cs:8,2246.2675912235)
--(axis cs:4,878.699773160089)
--cycle;
\addplot [semithick, blue]
table {%
4 1006.28293480123
8 1918.54556503313
16 3282.81462273275
32 4650.01829202252
};
\addplot [semithick, red]
table {%
4 1096.36288394545
8 2061.70022706192
16 3123.24112737846
32 3890.26078670246
};
\addplot [semithick, green]
table {%
4 992.430199191606
8 1988.90540678318
16 3943.68417650609
32 7000.1890459839
};
\addplot [semithick, color0]
table {%
4 1688.44894305017
8 3353.38973850364
16 5181.86558233608
32 6482.08089586539
};
\addplot [semithick, color1]
table {%
4 786.792488220836
8 1739.09898884838
16 3168.17134156203
32 4458.54838609967
};
\addplot [semithick, orange]
table {%
4 997.80610450189
8 2280.50258690287
16 3736.94115591646
32 5460.37118755587
};
\end{axis}

\end{tikzpicture}


==> fig/rate_by_environment/thesis_experiments_early_coverage_rate_2420f96.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0,0.811764705882353,1}
\definecolor{color0}{rgb}{0.12156862745098,0.227450980392157,0.00392156862745098}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Num. Robots},
xmin=2.6, xmax=33.4,
xtick style={color=black},
xtick={4,8,16,32},
xmajorgrids,
y grid style={lightgray!92.0261437908!black},
ylabel={Coverage Rate (cells per robot-iteration)},
ymin=0, ymax=650,
ymajorgrids,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,407.142081487262)
--(axis cs:8,335.591811535698)
--(axis cs:16,267.150269198492)
--(axis cs:32,184.64958567001)
--(axis cs:32,178.210478661895)
--(axis cs:16,257.254208767354)
--(axis cs:8,323.305861567847)
--(axis cs:4,380.966366751042)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,476.037986039159)
--(axis cs:8,387.66237287876)
--(axis cs:16,280.791426789792)
--(axis cs:32,184.84776198602)
--(axis cs:32,180.456812959203)
--(axis cs:16,268.967054584342)
--(axis cs:8,372.817656514502)
--(axis cs:4,461.552366018758)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,567.484220208668)
--(axis cs:8,511.198458445218)
--(axis cs:16,393.976196954534)
--(axis cs:32,279.771010842432)
--(axis cs:32,273.393693415613)
--(axis cs:16,384.563129754697)
--(axis cs:8,495.792393753133)
--(axis cs:4,538.599444790804)
--cycle;
\path [draw=color0, fill=color0, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,635.224325381101)
--(axis cs:8,507.09686740853)
--(axis cs:16,382.973709847493)
--(axis cs:32,249.113386833464)
--(axis cs:32,243.415566108141)
--(axis cs:16,374.600248705656)
--(axis cs:8,495.591288749075)
--(axis cs:4,618.121432303232)
--cycle;
\path [draw=color1, fill=color1, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,616.122685044893)
--(axis cs:8,572.573051020063)
--(axis cs:16,465.761246375949)
--(axis cs:32,348.44824618666)
--(axis cs:32,336.507969520028)
--(axis cs:16,448.478081381693)
--(axis cs:8,557.18547218301)
--(axis cs:4,597.112382246744)
--cycle;
\path [draw=orange, fill=orange, opacity=0.2, line width=0.0pt, dashed]
(axis cs:4,422.90783146409)
--(axis cs:8,326.24371036102)
--(axis cs:16,227.315975424154)
--(axis cs:32,135.344967540446)
--(axis cs:32,133.321993117212)
--(axis cs:16,222.890875335593)
--(axis cs:8,315.757226622667)
--(axis cs:4,397.508499630879)
--cycle;
\addplot [semithick, blue, dash pattern=on 3.7pt off 1.6pt]
table {%
4 394.054224119152
8 329.448836551772
16 262.202238982923
32 181.430032165953
};
\addplot [semithick, red, dash pattern=on 3.7pt off 1.6pt]
table {%
4 468.795176028959
8 380.240014696631
16 274.879240687067
32 182.652287472612
};
\addplot [semithick, green, dash pattern=on 3.7pt off 1.6pt]
table {%
4 553.041832499736
8 503.495426099176
16 389.269663354615
32 276.582352129022
};
\addplot [semithick, color0, dash pattern=on 3.7pt off 1.6pt]
table {%
4 626.672878842167
8 501.344078078803
16 378.786979276574
32 246.264476470803
};
\addplot [semithick, color1, dash pattern=on 3.7pt off 1.6pt]
table {%
4 606.617533645819
8 564.879261601537
16 457.119663878821
32 342.478107853344
};
\addplot [semithick, orange, dash pattern=on 3.7pt off 1.6pt]
table {%
4 410.208165547484
8 321.000468491844
16 225.103425379874
32 134.333480328829
};
\end{axis}

\end{tikzpicture}


==> fig/rate_by_environment/thesis_experiments_early_coverage_rate_per_iteration_2420f96.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0,0.811764705882353,1}
\definecolor{color0}{rgb}{0.12156862745098,0.227450980392157,0.00392156862745098}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black},
legend image post style={scale=0.5}, % resize legend entries
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Num. Robots},
xmajorgrids,
xmin=2.6, xmax=33.4,
xtick style={color=black},
xtick={4,8,16,32},
y grid style={lightgray!92.0261437908!black},
ylabel={Coverage Rate (cells per iteration)},
ymajorgrids,
ymin=0, ymax=12000,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.2, line width=0.0pt]
(axis cs:4,1628.56832594905)
--(axis cs:8,2684.73449228558)
--(axis cs:16,4274.40430717587)
--(axis cs:32,5908.78674144032)
--(axis cs:32,5702.73531718065)
--(axis cs:16,4116.06734027767)
--(axis cs:8,2586.44689254277)
--(axis cs:4,1523.86546700417)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0.0pt]
(axis cs:4,1904.15194415664)
--(axis cs:8,3101.29898303008)
--(axis cs:16,4492.66282863667)
--(axis cs:32,5915.12838355264)
--(axis cs:32,5774.61801469451)
--(axis cs:16,4303.47287334948)
--(axis cs:8,2982.54125211602)
--(axis cs:4,1846.20946407503)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0.0pt]
(axis cs:4,2269.93688083467)
--(axis cs:8,4089.58766756175)
--(axis cs:16,6303.61915127255)
--(axis cs:32,8952.67234695781)
--(axis cs:32,8748.59818929961)
--(axis cs:16,6153.01007607515)
--(axis cs:8,3966.33915002507)
--(axis cs:4,2154.39777916322)
--cycle;
\path [draw=color0, fill=color0, opacity=0.2, line width=0.0pt]
(axis cs:4,2540.89730152441)
--(axis cs:8,4056.77493926824)
--(axis cs:16,6127.57935755988)
--(axis cs:32,7971.62837867086)
--(axis cs:32,7789.29811546052)
--(axis cs:16,5993.60397929049)
--(axis cs:8,3964.7303099926)
--(axis cs:4,2472.48572921293)
--cycle;
\path [draw=color1, fill=color1, opacity=0.2, line width=0.0pt]
(axis cs:4,2464.49074017957)
--(axis cs:8,4580.5844081605)
--(axis cs:16,7452.17994201518)
--(axis cs:32,11150.3438779731)
--(axis cs:32,10768.2550246409)
--(axis cs:16,7175.64930210709)
--(axis cs:8,4457.48377746408)
--(axis cs:4,2388.44952898698)
--cycle;
\path [draw=orange, fill=orange, opacity=0.2, line width=0.0pt]
(axis cs:4,1691.63132585636)
--(axis cs:8,2609.94968288816)
--(axis cs:16,3637.05560678646)
--(axis cs:32,4331.03896129429)
--(axis cs:32,4266.30377975079)
--(axis cs:16,3566.25400536949)
--(axis cs:8,2526.05781298134)
--(axis cs:4,1590.03399852351)
--cycle;
\addplot [semithick, blue]
table {%
4 1576.21689647661
8 2635.59069241418
16 4195.23582372677
32 5805.76102931049
};
\addlegendentry{Boxes}
\addplot [semithick, red]
table {%
4 1875.18070411584
8 3041.92011757305
16 4398.06785099307
32 5844.87319912357
};
\addlegendentry{Hallway-Boxes}
\addplot [semithick, green]
table {%
4 2212.16732999894
8 4027.96340879341
16 6228.31461367385
32 8850.63526812871
};
\addlegendentry{Plane-Boxes}
\addplot [semithick, color0]
table {%
4 2506.69151536867
8 4010.75262463042
16 6060.59166842519
32 7880.46324706569
};
\addlegendentry{Empty}
\addplot [semithick, color1]
table {%
4 2426.47013458327
8 4519.03409281229
16 7313.91462206114
32 10959.299451307
};
\addlegendentry{Skylight}
\addplot [semithick, orange]
table {%
4 1640.83266218994
8 2568.00374793475
16 3601.65480607798
32 4298.67137052254
};
\addlegendentry{Office}
\end{axis}

\end{tikzpicture}

